Scalable Planning and Learning Framework Development for Swarm-to-Swarm Engagement Problems

Development of guidance, navigation and control frameworks/algorithms for swarms attracted significant attention in recent years. That being said, algorithms for planning swarm allocations/trajectories for engaging with enemy swarms is largely an understudied problem. Although small-scale scenarios can be addressed with tools from differential game theory, existing approaches fail to scale for large-scale multi-agent pursuit evasion (PE) scenarios. In this work, we propose a reinforcement learning (RL) based framework to decompose to large-scale swarm engagement problems into a number of independent multi-agent pursuit-evasion games. We simulate a variety of multi-agent PE scenarios, where finite time capture is guaranteed under certain conditions. The calculated PE statistics are provided as a reward signal to the high level allocation layer, which uses an RL algorithm to allocate controlled swarm units to eliminate enemy swarm units with maximum efficiency. We verify our approach in large-scale swarm-to-swarm engagement simulations.

==> referans.tex <==



==> sections/architecture.tex <==



\begin{figure}[H]
    \centering
    \includegraphics[width=\textwidth]{RL_figures/rl_arc_3.png}
    \caption{Arch}
    \label{fig:rl_arc}
\end{figure}


==> sections/problem_formulation.tex <==
\hspace{0.1cm}

Consider a multi-player pursuit-evasion game with a group of $n_p$ pursuer and $n_e$ evader agents in a bounded, convex environment $ Q \subset \mathbb{R}^{2}$ with points given as $q$. We assume all agents have the following equations of motion \cite{inter_rogue_robots} 

\begin{eqnarray}
\begin{split}
\dot{x}_e^i &= u_e^i, \quad \Vert u_e(t) \Vert \leq v_{\max },\\
\ \dot{x}_p^j &= u_p^j, \quad \Vert up(t) \Vert \leq v_{\max }, 
\label{eq:1}
\end{split}
\end{eqnarray}

where ${x}_e^i$ denote the positions of evaders for $i \in \{1,...,n_e\}$, ${x}_p^j$ denote the positions of pursuers for $j \in \{1,...,n_p\}$. ${u}_e$ and ${u}_p$ represent the control inputs of evaders and pursuers, respectively, and both subject to identical maximum velocity $v_{\max }$. We assume that $v_{\max} = 1$ for the rest of the paper. 

Define the capture condition of the evader $i$ at $x_e^i(t_c)$ for the pursuers as,

\begin{eqnarray} 
\min _{j \in n_p} \Vert x_e^i(t_c) - x_p^j(t_c) \Vert < r_c, \label{eq:2}
\end{eqnarray}

where $r_c > 0$ is the capture radius.

\subsection{Pursuit Strategies}
\subsubsection{Area-Minimization Policy}
In this section, we briefly describe the area-minimization policy for pursuers to capture an evader by decreasing its safe reachable area which is denoted as $A_e$, in consistent with the existing literature. $A_e$ is defined with points that the evader can reach before any other agent. Throughout the section, we adapt the notation used in \cite{inter_rogue_robots}.

Safe reachable area of the evader reduces to its Voronoi cell under the assumption of pursuers and evaders both having equal speeds. Voronoi tessellation is defined in \ref{eq:4}

\begin{eqnarray} 
V_i = \lbrace q \in Q | \Vert q - x^i \Vert \leq \Vert q - x^j \Vert, \forall j \ne i, \;\;i,j \leq n \rbrace. 
\label{eq:4}
\end{eqnarray}

The area of the Voronoi cell $V_e$ containing the evader is calculated as follows,

\begin{eqnarray} 
A_e = \int _{V_e} dq,
\label{eq:3}
\end{eqnarray}

The dynamics of $A_e$ are given by,

\begin{eqnarray}
\dot{A}_e = \frac{\partial A_e}{\partial x_e} \dot{x}_e + \sum _{j=1}^{n_p} \frac{\partial A_e}{\partial x_p^j} \dot{x}_p^j. 
\label{eq:5}
\end{eqnarray}

According to the given dynamics \eqref{eq:5}, pursuers cooperatively try to minimize the time derivative of $A_e$ while the evader try to maximize it as an opposite act of action. The joint objective for pursuers may reduce to minimization of each agent's individual contribution $\frac{\partial A_e}{\partial x_p^j} \dot{x}_p^j$. To lead pursuers in the direction of the fastest decrease of the evader's area, we define the control input for the pursuer $j$ as,

\begin{eqnarray} 
u_p^j = - \frac{\frac{\partial A_e}{\partial x_p^j}}{\Vert \frac{\partial A_e}{\partial x_p^j} \Vert }. 
\label{eq:6}
\end{eqnarray}

The gradient $\frac{\partial A_e}{\partial x_p^j}$ is calculated as,

\begin{eqnarray}
\frac{\partial A_e}{\partial x_p^j} = \frac{L_j}{\Vert x_p^j - x_e \Vert }\left(x_p^j - C_{b_j} \right).
\label{eq:7}
\end{eqnarray}

where $L_j$ is the area, $C_{b_j}$ is the centroid of the boundary. 
Details regarding the derivation of the gradient can be found in \cite{inter_rogue_robots}.

Substituting \eqref{eq:7} into \eqref{eq:6}, control policy of the pursuer reduces to

\begin{eqnarray}
u_p^j = \frac{\left(C_{b_j} - x_p^j \right)}{\Vert C_{b_j} - x_p^j \Vert }. 
\label{eq:8}
\end{eqnarray}

\subsubsection{Pure Distance Pursuit}
Pure-distance pursuit policy implies that a pursuer moves directly towards its nearest evader ${e}^\kappa$ of which $\kappa$ is determined from the expression\cite{inter_rogue_robots}

\begin{eqnarray}
\kappa = \text{arg min}_{i \in n_e}{\Vert x_{e}^\kappa - x_p^j \Vert }.
\label{eq:9}
\end{eqnarray}

Control policy is calculated as,

\begin{eqnarray} 
u_p^j = \frac{\left(x_{e}^\kappa - x_p^j \right)}{\Vert x_{e}^\kappa - x_p^j \Vert }. \label{eq:10}
\end{eqnarray}

\subsection{Evasion Strategies}
\subsubsection{Constant Area Policy}
Under the area-minimization strategy, the area $A_e$ is always non-increasing until the capture condition is met for any admissible control strategy\cite{inter_rogue_robots}. Only control policy that the evader can apply to keep the area constant is given as,

\begin{eqnarray}
u_e^* = \frac{\left(C_{b} - x_e \right)}{\Vert C_{b} - x_e \Vert },
\label{eq:11}
\end{eqnarray}

where $C_b$ indicates the middle point of the shared Voronoi boundary between pursuer $x_p$ and evader $x_e$.



\subsubsection{Move-to-centroid Policy}
In accordance with the \cite{inter_rogue_robots}
we choose to use move-to-centroid as one of the policies of the evader.

\begin{eqnarray} 
u_e^i = \frac{\left(C_{V_i} - x_e^i \right)}{\Vert C_{V_i} - x_e^i \Vert },
\label{eq:12}
\end{eqnarray}

where $V_i$ is the Voronoi region of the evader and $C_{V_i}$ is the centroid. Under this policy, evader can avoid not only one but multiple pursuers by moving towards the centroid and getting away from its cell's edges.



